Uncertainty-aware Consistency Learning for Cold-Start Item Recommendation

Graph Neural Network (GNN)-based models have become the mainstream approach for recommender systems. Despite the effectiveness, they are still suffering from the cold-start problem, i.e., recommend for few-interaction items. Existing GNN-based recommendation models to address the cold-start problem mainly focus on utilizing auxiliary features of users and items, leaving the user-item interactions under-utilized. However, embeddings distributions of cold and warm items are still largely different, since cold items' embeddings are learned from lower-popularity interactions, while warm items' embeddings are from higher-popularity interactions. Thus, there is a seesaw phenomenon, where the recommendation performance for the cold and warm items cannot be improved simultaneously. To this end, we proposed a Uncertainty-aware Consistency learning framework for Cold-start item recommendation (shorten as UCC) solely based on user-item interactions. Under this framework, we train the teacher model (generator) and student model (recommender) with consistency learning, to ensure the cold items with additionally generated low-uncertainty interactions can have similar distribution with the warm items. Therefore, the proposed framework improves the recommendation of cold and warm items at the same time, without hurting any one of them. Extensive experiments on benchmark datasets demonstrate that our proposed method significantly outperforms state-of-the-art methods on both warm and cold items, with an average performance improvement of 27.6%.

==> 1to2.preli.tex <==
\section{Preliminaries}\label{sec::probdef}
% In this section, we introduce notations and formulate the problem.
% We then 
% \noindent\textbf{Notations and Problem Overview.}
\subsection{Problem Formulation}
%\chenc{we should emphasize long-tail recommendation here;}
\noindent\textbf{Notations.} The common GNN-based model paradigm can be formulated as follows: Let $\mathcal{U}=\{u\}$, $\mathcal{I}=\{i\}$ denote the set of users and items respectively. The interactions of user and item can be regard as $\mathcal{O}=\left\{(u, i^{+}) \mid u \in \mathcal{U}, i^{+} \in \mathcal{I}\right\}$, where each pair shows each observed feedback.

\noindent\textbf{Input:} Most GNN-based models treat user-item interactions as a bipartite graph, where the node set is $\mathcal{V} = \mathcal{U} \cup \mathcal{I}$ and the edge set is $\mathcal{G} = (\mathcal{V}, \mathcal{O}^{+})$. In the training process of graph representation learning, we use $\textbf{E}_u = [e_{u_{1}},\cdots,e_{u_{M}}]\in \mathbb{R}^{M \times D}, \textbf{E}_i = [e_{i_{1}},\cdots,e_{i_{N}}]\in \mathbb{R}^{N \times D}$ 
to denote the user embedding and item embedding, where D is the dimension size of embedding, $M, N$ are the number of users and items respectively.

\noindent\textbf{Output:} Usually, the top-k items in the ranking list are selected as the recommended items. Specifically, recommender models estimate the scores $S_m = \{s_{mn}\}_{n=1}^{n=N}$ of all items for each user $u_m$, where $s_{mn}$ is calculated as:
\begin{equation}
    s_{mn} = e_{u_{m}}e_{i_{n}}^T
\end{equation}
then rank items by their scores - a high score means that the user prefers. The top-k items from the ranking list are adopted into a candidate set and recommended to the user. The recall process for each user can be formulated as:
\begin{equation}
    \widehat{\mathcal{I}}_\textbf{candidate}= \text{Top-K}(S_m)
\end{equation}



==> 4.related.tex <==
\section{Related Work}\label{sec::related}


\textbf{Recommender systems} aim to provide personalized content and services by utilizing user-item interaction history and help people filter, prioritize, deliver precise information in the era of the Internet. A large number of recommendation systems \cite{he2016fast, he2017neural} are based on collaborative filtering (CF), which makes predictions according to the similarity of historical choice among users.

%With the development of the Internet, people are suffering the problem of information overload and choice overwhelming. How to filter, prioritize and efficiently deliver precise information becomes a big challenge. To solve this problem, recommender system  provides personalized content and services by utilizing user-item interaction history. 

Recent years, with the development of deep learning, graph neural network (GNN) based recommendation methods \cite{wang2020multi, wang2020disentangled, wu2020joint, wu2019session, wu2020learning} have developed rapidly. They bring GNNs into CF. In the matching stage, GNN based model can be regarded as embedding matching, then user-item interactions can be naturally modeled in the form of a bipartite graph to capture higher-order information. For example, Pinsage \cite{ying2018graph} uses random walk to sample neighbors and the sampled counts are regard as the important coefficients when performing neighborhood aggregation. GCMC \cite{berg2017graph} designs a graph-based auto-encoder to aggregate adjacency information. NGCF \cite{he2017neural} captures high-order similarity among users and items to improve embedding learning. And LightGCN \cite{he2020lightgcn} further simplifies neighborhood aggregation by removing transformation matrix.

Based on these models, some techniques \cite{berg2017graph, rong2019dropedge} have also been applied to improve the recommendation performance. KGAT \cite{wang2019kgat} introduces knowledge graph and utilize attention mechanism to exploit high-order relationships. SGL \cite{wu2021self} leverages the stability of graph structure to incorporate a contrastive learning framework. RecEraser \cite{chen2022recommendation} proposes a machine unlearning framework to forget part of the learned data for the model robustness. However, these methods overlook the long-tail problem of recommendation data, which restricts their performance. 

% with less emphasize on the long-tail distribution

\noindent \textbf{The long-tail problem} is very common in the real world, like computer vision \cite{gupta2019lvis} and recommendation. In the recommendation area, the long-tail distribution of user feedback is quite obvious, especially on the item side. Some studies focus on tail items to improve the tail item recommendation. For example, Inverse Propensity Score (IPS) methods \cite{schnabel2016recommendations, yang2018unbiased} re-weight the scores of tail items with their popularity, and clustering methods \cite{park2012adaptive, park2008long} find similar items for wider recommendations. TailNet \cite{liu2020long} designs learnable rectification factors to softly balance the representation of head items and tail items. In addition, some studies also try to transfer the knowledge from head nodes to tail nodes. Meta-tail2vec \cite{liu2020towards} builds a regression problem to learn tail node embeddings by using the rich structural information in high-degree nodes. TailGNN \cite{liu2021tail} learns a neighborhood translation from the structurally rich head nodes and transfers the knowledge to the structurally limited tail. MIRec \cite{zhang2021model} transfers knowledge from head items that contain rich user feedback information to help learn tail items in the long-tail distribution problem. The cold start problem can also be regard as a long-tail problem. These recommenders \cite{zheng2021multi, volkovs2017dropoutnet, lee2019melu} usually leverage side information such as user profile and content information to enhance the representation learning of tail items. 

% In recommendation, a large amount of real user data is collected and distributed in a long tail.  and Resampling the  to reach the unbiased performance. With the development of deep learning, some advanced techniques are used to solve the long tail problem. Some recent works used tranfer learning  transfer the knowledge of head and tail nodes to complement each other to achieve better results.

% GNN-based models are designed to comprehensively learn long-tail relationships in the form of graphs.

\noindent \textbf{Self-training} \cite{scudder1965probability, riloff1996automatically, riloff2003learning} is a training approach that has been widely investigated in semi-supervised learning. Recently, with the development of deep learning, self-training has made great success in areas like computer vision \cite{xie2020self, sohn2020fixmatch, wang2021data}, natural language processing \cite{he2019revisiting} and speech processing \cite{kahn2020self, parthasarathi2019lessons}. For these tasks, usually a certain amount of labeled samples and a large number of unlabeled data are available. The goal is to utilize the large unlabeled data to boost performance. The practice is to utilize pseudo labels \cite{lee2013pseudo}. Specifically,  a teacher model is trained on the labeled data. Then, it performs inference on the unlabeled samples to obtain pseudo labels. The pseudo labels are then regarded as their ground-truth for training the subsequent model called the student model. %With more training data participating in, the student model usually holds a better performance than the teacher model.
% In recommendations, recent studies using side information to generate ground-truth samples from raw data to learn robust representation. 

The advantage of self-training is that it is able to utilize more training data, but does not require extra human efforts to annotate them. Because of this, recent works have resorted self-training to solve the data scarcity and the long-tail problem in recommendations. For example, SEPT \cite{yu2021socially} generates pseudo labels with the help of social networks to improve the recommendation performance. In the session recommendation scenario, by building two homogeneous graphs from item view and session view, COTREC \cite{xia2021self} trains two encoders from different views with their generated pseudo labels. Saito \emph{et al.} \cite{saito2020asymmetric} pre-trains three recommendation models and takes out two of them to provide pseudo labels for predicting the truly recommendation results without selection bias. 

However, existing works usually require side information (e.g. social network, session information) or need multiply models to provide pseudo labels, which is information missing and space consuming. Differently, we only leverage user-item interactions for building a bipartite graph and just need one model for pseudo label generation.  
